PlanGPT: Enhancing Urban Planning with Tailored Language Model and Efficient Retrieval

In the field of urban planning, general-purpose large language models often struggle to meet the specific needs of planners. Tasks like generating urban planning texts, retrieving related information, and evaluating planning documents pose unique challenges. To enhance the efficiency of urban professionals and overcome these obstacles, we introduce PlanGPT, the first specialized Large Language Model tailored for urban and spatial planning. Developed through collaborative efforts with institutions like the Chinese Academy of Urban Planning, PlanGPT leverages a customized local database retrieval framework, domain-specific fine-tuning of base models, and advanced tooling capabilities. Empirical tests demonstrate that PlanGPT has achieved advanced performance, delivering responses of superior quality precisely tailored to the intricacies of urban planning.

==> figure_n_table/Format.tex <==
\begin{table*}[htbp]
\centering
\begin{tabularx}{\textwidth}{l|X}
\hline
\textbf{Type}    & \textbf{Fine-tuning format}   \\ \hline
Short-answer questions (\begin{CJK*}{UTF8}{gbsn}简答题\end{CJK*}) & \{\begin{CJK*}{UTF8}{gbsn}{"Q":"人地相关论是什么? ",
 "A":"人地相关论是20世纪20年代法国近代人文地理学的奠基人白兰士所倡导的理论。在人地关系中，白兰士反对拉采尔的环境决定论思想，他认为，除了环境的直接影响外，还有其他因素在起作用，强调人类对外界环 境的适应不是被动的而是主动的，因而人与自然环境之间是相互作用的，他的理论被称为"人地相关论"。法国的人地相关论思想使人地关系理论研究有了很大的进步。"}\end{CJK*}\}                                         \\ \hline
Summary questions  (\begin{CJK*}{UTF8}{gbsn}综述题\end{CJK*})   &  \{\begin{CJK*}{UTF8}{gbsn} {"Q":"为什么说人地关系研究是人文地理学研究的核心课题?"
  "A":"(1)人地关系是一种普遍存在的客观关系，是人文地理学研究的中心课题，也是人文地理学重要的理论基础。(2)人地关系研究是人文地理学研究的核心课题: 人文地理学是研究地表人文事象的空间分布及其空间差别，并预测其发展和变化规律的科学，它是以人地关系为基础，着重于地表人类活动或人与环境所形成的各种文化现象的分布与变化。...... 人文地理学研究人地关系必须以环境为基础，脱离了地，也就不能称其为地理学研究。人和地是矛盾的统一体，人文地理学需要用生态学的规律，主动协调人类活动与自然环境之间的关系，预测人类活动可能引起的变化和后果，在开发利用的同时优化人类的生态环境。"} \end{CJK*}                                      \\ \hline
Essay questions (\begin{CJK*}{UTF8}{gbsn}文本题\end{CJK*}) &   \{\begin{CJK*}{UTF8}{gbsn} { "Q": "成都市国土空间总体规划2020-2035的主要内容是什么？",
  "A": "主要内容包括：\n1. 战略定位：建设国家中心城市、美丽宜居公园城市、国际门户枢纽城市、世界文化名城，迈向充分体现中国特色、时代特征、成都特质的可持续发展世界城市。\n2. 城市职能：规划中明确了成都作为全国重要的经济中心、科技中心、金融中心、文创中心、对外交往中心的城市定位，还强调了其作为国际性综合交通通信枢纽的地位。\n3. 发展目标：规划设定了发展目标，包括在2025年建设为全国重要的经济、科技、金融、文创、对外交往中心和国际综合交通通信枢纽城市，基本建成践行新发展理念的公园城市示范区。"} \end{CJK*}     \\ \hline
\end{tabularx}
\caption{Question type and format. }

%% 格式需要修正
\text{Short-answer questions provide rich knowledge in geography and planning from foundational textbooks, while summary questions enhance domain-specific thinking abilities through geography and planning exam questions. Essay questions cultivate expertise in the official planning text style by drawing from government documents.}


\label{format}
\end{table*}









